Multi-resolution Tensor Learning for Large-Scale Spatial Data

High-dimensional tensor models are notoriously computationally expensive to train. We present a meta-learning algorithm, MMT, that can significantly speed up the process for spatial tensor models. MMT leverages the property that spatial data can be viewed at multiple resolutions, which are related by coarsening and finegraining from one resolution to another. Using this property, MMT learns a tensor model by starting from a coarse resolution and iteratively increasing the model complexity. In order to not "over-train" on coarse resolution models, we investigate an information-theoretic fine-graining criterion to decide when to transition into higher-resolution models. We provide both theoretical and empirical evidence for the advantages of this approach. When applied to two real-world large-scale spatial datasets for basketball player and animal behavior modeling, our approach demonstrate 3 key benefits: 1) it efficiently captures higher-order interactions (i.e., tensor latent factors), 2) it is orders of magnitude faster than fixed resolution learning and scales to very fine-grained spatial resolutions, and 3) it reliably yields accurate and interpretable models.

==> sec-abstract.tex <==
\begin{abstract}

We present a meta-learning algorithm to efficiently learn both accurate and interpretable spatial latent factor models from high-resolution data.
Our method learns using multiple resolutions, by starting from a low resolution model and adaptively increasing the model complexity, and is compatible with any gradient-based optimizer.
%
In order to not "over-train" on low-resolution models, our approach also uses early stopping criteria to choose when to transition to higher-resolution models.
%
We showcase our method on two real-world datasets for basketball tracking and animal behavior, and demonstrate 3 key benefits of our approach: 1) it reliably yields accurate and interpretable models, 2) it scales to very fine-grained models with higher-order interactions (i.e., tensor latent factor models), and 3) it can be an order of magnitude faster than fixed resolution training.
%
\end{abstract}

